GUISE: Graph GaUssIan Shading watErmark

In the expanding field of generative artificial intelligence, integrating robust watermarking technologies is essential to protect intellectual property and maintain content authenticity. Traditionally, watermarking techniques have been developed primarily for rich information media such as images and audio. However, these methods have not been adequately adapted for graph-based data, particularly molecular graphs. Latent 3D graph diffusion(LDM-3DG) is an ascendant approach in the molecular graph generation field. This model effectively manages the complexities of molecular structures, preserving essential symmetries and topological features. We adapt the Gaussian Shading, a proven performance lossless watermarking technique, to the latent graph diffusion domain to protect this sophisticated new technology. Our adaptation simplifies the watermark diffusion process through duplication and padding, making it adaptable and suitable for various message types. We conduct several experiments using the LDM-3DG model on publicly available datasets QM9 and Drugs, to assess the robustness and effectiveness of our technique. Our results demonstrate that the watermarked molecules maintain statistical parity in 9 out of 10 performance metrics compared to the original. Moreover, they exhibit a 100% detection rate and a 99% extraction rate in a 2D decoded pipeline, while also showing robustness against post-editing attacks.

==> sections/progress_w3.tex <==
\section{progress week 3}
watermark embedding/extracting in latent space \\
\includegraphics[width=0.8\textwidth]{research paper/images/week4_img.png} \\
blue line: embedding, red line: extracting \\
encryption/decryption: Chacha20, a steam cipher for the symmetric key. (due to the security property of the ciphertext, we can assume that in the cipher text each bit have equal property to become 1 or 0) \\


\begin{verbatim}
embedding: Latent[i] = norm.ppf((ciphertextbits[i] + np.random.uniform(0,1)) / 2)
extracting: ciphertextbits[i] = int(norm.cdf(Latent[i]) * 2)
\end{verbatim}


\includegraphics[width=0.8\textwidth]{research paper/images/week4_img2.png} \\
we can assume the watermark method generates a (pseudo)random gaussian


However, DDIM and DDIM-inverse are deterministic but not reversable. encoder and decoder are deterministic but only one way reversible. see blow diagram


==> sections/responsible_research.tex <==
\section{Responsible Research}
\lc{Put it at the very end. Not important}
This study strictly adheres to ethical guidelines with all datasets being sourced from Nature under a CC BY license, ensuring open and accessible data use. The autoencoder and diffusion models used in this study were provided by the authors of LDM-3DG under the GPL-3.0 license. Additionally, the Gaussian Shading method and its implementation are under the MIT License. No potential conflicts of interest were identified in this study. Detailed methodologies and all original data and code are available for replication purposes on GitLab: \url{https://gitlab.ewi.tudelft.nl/dmls/courses/cse3000/watermark/graph-diffusion}.

%\je{Better to show the URL in a footnote. Right now it is unclear that this is an ULR.}

==> sections/your_contribution.tex <==
\section{Evaluation}
In computer science typically the third section contains an exposition of the main ideas, for example, the development of a theory, the analysis of the problem (some proofs), a new algorithm, and potentially some theoretical analysis of the properties of the algorithm.

Do not forget to give this section another name, for example after the method or idea you are presenting.

Some more detailed suggestions for typical types of contributions in computer science are described in the following subsections.


\subsection*{Experimental work}
In this case, this section will mostly contain a description of the methods/algorithms you will be comparing. Although not all methods need to be described in detail (providing appropriate references are available), make sure that you reveal sufficient details to a reader not familiar with these methods to: a) obtain a high-level understanding of the method and differences between them, and b) understand your explanation of the results/conclusions.

\subsection*{Improvement of an idea}
In this case, you would need to explain in detail how the improvement works. If it is based on some observation that can be proven, this is a good place to provide that proof (e.g., of the correctness of your approach). 

\subsection*{Literature survey}
If your contribution is a literature survey, then the organization of these ``middle'' sections very much depends on the way you want to present/organize the literature you are discussing.
First, try to cluster papers that are similar in some aspect. Then think of how these clusters are related, from that you can think of a good order to discuss these clusters; this is sometimes called a bottom-up approach to writing a paper.

In addition, you may try to think about the organization of the literature from a top-down perspective: try to ``take a step back'' and think about the field and what important questions/variants are and build a hierarchical categorization of the field.

Make clear what your contribution is here: a new organization of the literature, identification of open problems/challenges, new parallels/generalizations, a table with pros/cons of different methods, etc.\ 


